A Unified Prediction Framework for Signal Maps

Signal maps are essential for the planning and operation of cellular networks. However, the measurements needed to create such maps are expensive, often biased, not always reflecting the metrics of interest, and posing privacy risks. In this paper, we develop a unified framework for predicting cellular signal maps from limited measurements. Our framework builds on a state-of-the-art random-forest predictor, or any other base predictor. We propose and combine three mechanisms that deal with the fact that not all measurements are equally important for a particular prediction task. First, we design quality-of-service functions ($Q$), including signal strength (RSRP) but also other metrics of interest to operators, i.e., coverage and call drop probability. By implicitly altering the loss function employed in learning, quality functions can also improve prediction for RSRP itself where it matters (e.g., MSE reduction up to 27% in the low signal strength regime, where errors are critical). Second, we introduce weight functions ($W$) to specify the relative importance of prediction at different locations and other parts of the feature space. We propose re-weighting based on importance sampling to obtain unbiased estimators when the sampling and target distributions are different. This yields improvements up to 20% for targets based on spatially uniform loss or losses based on user population density. Third, we apply the Data Shapley framework for the first time in this context: to assign values ($\phi$) to individual measurement points, which capture the importance of their contribution to the prediction task. This improves prediction (e.g., from 64% to 94% in recall for coverage loss) by removing points with negative values, and can also enable data minimization. We evaluate our methods and demonstrate significant improvement in prediction performance, using several real-world datasets.

==> tables/methodology-overview.tex <==
\begin{table*}
		  \centering
	\setlength\tabcolsep{1.5pt} % default value: 6pt
	\caption{ Overview of the Methodologies in this paper: (i) Input handling with Importance sampling and (ii) Custom Network Quality Functions/ Loss Functions to \emph{align} with the Mobile Network Carriers (MNCs) objectives.}
	\vspace{-5pt}
	\label{tab:customfunctions+_methodology}
	%\scriptsize
	\begin{tabular}{|l|l|l|l|}
		\hline
		\textbf{MNCarrier Objective}                                                                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}(1/3) Custom Loss Function,        \\         Explicit Training\end{tabular}}                      & \textbf{(2/3) Weighted Random Forests} & \textbf{\begin{tabular}[c]{@{}l@{}}(3/3) Implicit Training on \\ Network Quality Function $Q(y)$\end{tabular}} \\ \hline
		\begin{tabular}[c]{@{}l@{}}a. Optimize Coverage:\\     Weak Reception Areas/Samples\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}$L_y^c (\widehat{y})$ $\rightarrow$ \\  (i) modified Hinge Loss\\  (ii) Huber Assymetric Loss\end{tabular} & $w_c$                                  & Coverage $Q_c(\widehat{P})$ \vs $\widehat{Q}(P)$                                                               \\ \hline
		\begin{tabular}[c]{@{}l@{}}b. Optimize Network Quality Function:\\     \eg Call Drop Probability\end{tabular}                                      & $L_y^{cdp} (\widehat{y})$ $\rightarrow$ exponential loss                                                                              & $w_{cdp} \leftarrow Q_{cdp}(y)$        & CDP $Q_{cdp}(\widehat{y})$ \vs  $\widehat{Q}(y)$                                                               \\ \hline
		\begin{tabular}[c]{@{}l@{}}c. Optimize on Measurement Density:\\    \eg Under sampled areas should be \\    considered equally.\end{tabular}       & $L_y^{d} (\widehat{y})$                                                                                                               & $w_c \leftarrow \frac{f_{kde}}{f_u}$   & \multirow{2}{*}{}                                                                                              \\ \cline{1-3}
		\begin{tabular}[c]{@{}l@{}}d. Optimize on Locations\\     of Interest: \eg Population density\\     based or 911 locations/hospitals.\end{tabular} & $L_y^{\vec{l}} (\widehat{y})$                                                                                                         & $w_{\vec{l}}$                          &                                                                                                                \\ \hline
	\end{tabular}
\end{table*}

==> tables/methodology-overview_v0.tex <==
\begin{table*}
		  \centering
	\setlength\tabcolsep{1.5pt} % default value: 6pt
	\caption{ Overview of the Methodologies in this paper: (i) Input handling with Importance sampling and (ii) Custom Network Quality Functions/ Loss Functions to \emph{align} with the Mobile Network Carriers (MNCs) objectives.}
	\vspace{-5pt}
	\label{tab:customfunctions+_methodology}
	%\scriptsize
	\begin{tabular}{|l|l|l|l|}
		\hline
		\textbf{MNCarrier Objective}                                                                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}(1/3) Custom Loss Function,        \\         Explicit Training\end{tabular}}                      & \textbf{(2/3) Weighted Random Forests} & \textbf{\begin{tabular}[c]{@{}l@{}}(3/3) Implicit Training on \\ Network Quality Function $Q(y)$\end{tabular}} \\ \hline
		\begin{tabular}[c]{@{}l@{}}a. Optimize Coverage:\\     Weak Reception Areas/Samples\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}$L_y^c (\widehat{y})$ $\rightarrow$ \\  (i) modified Hinge Loss\\  (ii) Huber Assymetric Loss\end{tabular} & $w_c$                                  & Coverage $Q_c(\widehat{P})$ \vs $\widehat{Q}(P)$                                                               \\ \hline
		\begin{tabular}[c]{@{}l@{}}b. Optimize Network Quality Function:\\     \eg Call Drop Probability\end{tabular}                                      & $L_y^{cdp} (\widehat{y})$ $\rightarrow$ exponential loss                                                                              & $w_{cdp} \leftarrow Q_{cdp}(y)$        & CDP $Q_{cdp}(\widehat{y})$ \vs  $\widehat{Q}(y)$                                                               \\ \hline
		\begin{tabular}[c]{@{}l@{}}c. Optimize on Measurement Density:\\    \eg Under sampled areas should be \\    considered equally.\end{tabular}       & $L_y^{d} (\widehat{y})$                                                                                                               & $w_c \leftarrow \frac{f_{kde}}{f_u}$   & \multirow{2}{*}{}                                                                                              \\ \cline{1-3}
		\begin{tabular}[c]{@{}l@{}}d. Optimize on Locations\\     of Interest: \eg Population density\\     based or 911 locations/hospitals.\end{tabular} & $L_y^{\vec{l}} (\widehat{y})$                                                                                                         & $w_{\vec{l}}$                          &                                                                                                                \\ \hline
	\end{tabular}
\end{table*}

==> tables/methodology-overview_v1.tex <==
\begin{table}
	\centering
	\setlength\tabcolsep{1.5pt} % default value: 6pt
	\caption{ \footnotesize  Quality Functions Domain-Methodology.}
	\vspace{-5pt}
	\label{tab:customfunctions_methodology_v2}
	\scriptsize
	\begin{tabular}{|l|l|l|}
		\hline
		\textbf{Training Options}               & \textbf{$y$ Domain}                                & \textbf{$Q(y)$ Domain}   \\ \hline \hline
		\textbf{$w_i = 1,  \forall i$ (Default)}          & $\widehat{y} \rightarrow$ $Q_{cdp}(\widehat{y})$   & $\widehat{Q}_{cdp}(y)$   \\ \hline
		\textbf{$w_i = \{w_u, w_P\}$ (See Tab.3)} & $\widehat{y} \rightarrow$ $Q^w_{cdp}(\widehat{y})$ & $\widehat{Q}^w_{cdp}(y)$ \\ \hline
	\end{tabular}
	\vspace{-20pt}
\end{table}


\iffalse

	\begin{tabular}{llll}
	\hline
	\multicolumn{2}{|l|}{\textbf{}}                                      & \multicolumn{1}{l|}{\textbf{Input}}                                                                                                                                                                                                                                 & \multicolumn{1}{l|}{\textbf{Output}}                                                                                                                                                           \\ \hline
	\multicolumn{2}{|l|}{\multirow{2}{*}{\textbf{Data $(x_i,y_i)$}}}     & \multicolumn{1}{l|}{Features $\mathbf{x}$}                                                                                                                                                                                                                          & \multicolumn{1}{l|}{KPIs  $y_i= \{y^P_i,y^I_i,y^C_i\}$}                                                                                                                                        \\ \cline{3-4} 
	\multicolumn{2}{|l|}{}                                               & \multicolumn{1}{l|}{$ \mathbf{x_i^{full}} = (l_i^x, l_i^y , d, h, \text{\cid}, \text{\dev}, out, ||\vec{l}_{BS} - \vec{l}_j ||_2, \text{\freq})$}                                                                                                                   & \multicolumn{1}{l|}{$y^P$: RSRP, $y^I$: RSRQ, $y^C$: CQI, $Q(y)$: Quality Function}                                                                                                            \\ \hline
	\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                \\ \hline
	\multicolumn{2}{|l|}{\multirow{3}{*}{\textbf{MNCarrier Objectives}}} & \multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Certain $\mathbf{x}_i$ are more important. \\ e.g. $\mathbf{x}_i$ with 911, hospital locations $\mathbf{l}_i$.\\ e.g. $\mathbf{x}_i$ with higher population $P(\mathbf{l}_i)$ etc.\end{tabular}}}    & \multicolumn{1}{l|}{(1) \textbf{Optimize} $\widehat{y}$ for certain input $\mathbf{x}_j$}                                                                                                      \\ \cline{4-4} 
	\multicolumn{2}{|l|}{}                                               & \multicolumn{1}{l|}{}                                                                                                                                                                                                                                               & \multicolumn{1}{l|}{(2) \textbf{Optimize} Coverage $Q_c(y)$ or Signal Bars $Q_B(y)$}                                                                                                           \\ \cline{4-4} 
	\multicolumn{2}{|l|}{}                                               & \multicolumn{1}{l|}{}                                                                                                                                                                                                                                               & \multicolumn{1}{l|}{(3) \textbf{Optimize} Call Drop Probability $Q_{cdp}(y)$}                                                                                                                  \\ \hline
	\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                \\ \hline
	\multicolumn{2}{|l|}{\textbf{Current Approaches:}}                   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(i) All $\mathbf{x}_i$ are equally weighted (e.g. cross-validation error).\\ (ii) Sampling miss-matches target distribution : $s(\mathbf{x}) != p(\mathbf{x})$.\end{tabular}}                                        & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(i) Optimize only  MSE.\\ (ii) Minimize only $\widehat{y}$\end{tabular}}                                                                        \\ \hline
	\multicolumn{2}{|l|}{\textbf{Our Methodology:}}                      & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Importance Sampling Framework $W(\mathbf{x})$:\\ (i) Adjusted errors $\varepsilon_p(y,\widehat{y})$ per target distribution $p(\mathbf{x})$.\\ (ii) Importance ratio weights $w_i$ for model training.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Network Quality Functions of Interest:\\ (i) $\widehat{Q}(y)$ vs. $Q(\widehat{y})$\\ (ii) $\widehat{Q}^w(y)$ vs. $\widehat{Q}(y)$\end{tabular}} \\ \hline
\end{tabular}
\fi

==> tables/table-TAIs-details.tex <==
\begin{table}
	  \centering
	\setlength\tabcolsep{1.5pt} % default value: 6pt
	\caption{\externalcitiesdataset: LTE TAs Examples.}
	\vspace{-5pt}
	\label{tab:LTE_TAs_Details}
	\scriptsize
	\begin{tabular}{|l||l|l|l|}
		\hline
		& \begin{tabular}[c]{@{}l@{}}NYC (MNC-1) \\ Manhattan Midtown\end{tabular} & \begin{tabular}[c]{@{}l@{}}NYC (MNC-1)\\ E. Brooklyn\end{tabular} & \begin{tabular}[c]{@{}l@{}}LA (MNC-2) \\ Southern\end{tabular} \\ \hline \hline
		No. Measurements                & $\approxeq 63$K                                                          & $\approxeq 104$K                                                  & $\approxeq 20$K                                                \\ \hline
		Area $km^2$                     & 1.8$km^2$ (Fig. 1 (c-d))                                                 & 44.8 $km^2$                                                       & 220 $km^2$                                                     \\ \hline
		Data Density $\frac{N}{m^2}$    & $\approxeq 0.035$                                                        & $\approxeq 0.002$                                                 & $\approxeq 0.0001$                                             \\ \hline
		No. Cells $|C|$                 & 429                                                                      & 721                                                               & 353                                                            \\ \hline
		Cell Density $\frac{|C|}{km^2}$ & 238.3                                                                    & 16.1                                                              & 1.6                                                            \\ \hline
	\end{tabular}
	\vspace{-10pt}
\end{table}
